Hydra: Bidirectional State Space Models Through Generalized Matrix Mixers

A wide array of sequence models are built on a framework modeled after Transformers, comprising alternating sequence mixer and channel mixer layers. This paper studies a unifying matrix mixer view of sequence mixers that can be conceptualized as a linear map on the input sequence. This framework encompasses a broad range of well-known sequence models, including the self-attention of Transformers as well as recent strong alternatives such as structured state space models (SSMs), and allows understanding downstream characteristics such as efficiency and expressivity through properties of their structured matrix class. We identify a key axis of matrix parameterizations termed sequence alignment, which increases the flexibility and performance of matrix mixers, providing insights into the strong performance of Transformers and recent SSMs such as Mamba. Furthermore, the matrix mixer framework offers a systematic approach to developing sequence mixers with desired properties, allowing us to develop several new sub-quadratic sequence models. In particular, we propose a natural bidirectional extension of the Mamba model (Hydra), parameterized as a quasiseparable matrix mixer, which demonstrates superior performance over other sequence models including Transformers on non-causal tasks. As a drop-in replacement for attention layers, Hydra outperforms BERT by 0.8 points on the GLUE benchmark and ViT by 2% Top-1 accuracy on ImageNet.

==> fig/quasi_corollary.tex <==
\begin{wrapfigure}{r}{0.31\textwidth}
\begin{minipage}{1.\linewidth}
\vspace{-4mm}
\includegraphics[width=\linewidth]{fig_img/quasi_corollary.pdf}
\centering
\vspace{-8mm}
\caption{
\textcolor{blue}{(Top) A mixer matrix of addition-based bidirectional SSMs. (Bottom) A quasiseparable matrix mixer for \name{}. The freedom in the diagonal values leads to a higher expressivity compared to mixer matrices of naive addition-based bidirectional SSMs, where the diagonal values are constrained by the colored vectors.}
\AG{As discussed in slack: (i) can maybe get rid of $A_{i:i}^\times$, to be more consistent here, but optional (ii) you can outline the below-diagonal and above-diagonal low-rank boxes as an illustration of the QS condition. (iii) think about the caption that explains the generalization proeprty, e.g. "(Top) QS matrices are characterized by a rank condition (Definition 3.1); (Bottom) because of a similar rank property for semiseparable matrices, an addition based bidirectional SSM is provably a quasiseparable matrix. Hence, QS matrix mixers generalize this common heuristic for bidirectional SSMs" Note that for a caption like this, it would make sense to swap the order of the two matrices to make it flow better}
}
\vspace{-30mm}
\label{fig:quasi_corollary}
\end{minipage}
\end{wrapfigure}


==> old_tab/abl_bi_graph.tex <==
\begin{wrapfigure}{r}{0.54\textwidth}
\begin{minipage}{1.\linewidth}
\vspace{-9mm}
\begin{figure}[H]
\centering
\begin{tikzpicture}[scale=1.0]
\begin{axis}[
    width=8cm,
    height=5cm,
    % title={Boundary AP vs. IoU thres.},
    xlabel={Training Steps (K)},
    x label style={at={(axis description cs:0.5,0.03)},anchor=north},
    % ylabel={Cross Entropy},
    xmin=10, xmax=71,
    ymin=1.65, ymax=2.0,
    xtick={0, 10, 20, 30, 40, 50, 60, 70},
    ytick={1.7, 1.8, 1.9, 2.0},
    legend pos=north east,
    ymajorgrids=true,
    grid style=dashed,
]
% \addplot[
%     color=black,
%     mark=square,
%     ]
%     coordinates {
%     (2, 4.7)(4, 4.14)(6, 3.938)(8, 3.841)(10, 3.779)(12, 3.734)(14, 3.7)(16, 
%     };
%     \addlegendentry{Uni}
\addplot[
    color=Indigo7,
    mark=square*,
    mark options={scale=0.7},
    ]
    coordinates {
    (2, 3.684)(4, 2.67)(6, 2.337)(8, 2.198)(10, 2.114)
    (12, 2.056)(14, 2.014)(16, 1.98)(18, 1.954)(20, 1.928)
    (22, 1.91)(24, 1.894)(26, 1.877)(28, 1.864)(30, 1.852)
    (32, 1.84)(34, 1.831)(36, 1.818)(38, 1.809)(40, 1.802)
    (42, 1.793)(44, 1.784)(46, 1.778)(48, 1.769)(50, 1.763)
    (52, 1.757)(54, 1.75)(56, 1.743)(58, 1.741)(60, 1.734)
    (62, 1.728)(64, 1.721)(66, 1.718)(68, 1.715)(70, 1.711)

    % 1.757 1.75    1.743   1.741   1.734   1.728   1.721   1.718   1.715   1.711
    % 1.754 1.748   1.74    1.739   1.733   1.727   1.72    1.717   1.714   1.71
    % 1.726 1.72    1.712   1.711   1.705   1.698   1.692   1.689   1.686   1.682
    % 1.71  1.703   1.697   1.694   1.689   1.683   1.677   1.674   1.671   1.667
    };
    \addlegendentry{Concat}
\addplot[
    color=Green7,
    mark=triangle*,
    mark options={scale=1.0},
    ]
    coordinates {
    (2, 3.575)(4, 2.649)(6, 2.323)(8, 2.185)(10, 2.103)
    (12, 2.047)(14, 2.005)(16, 1.972)(18, 1.946)(20, 1.921)
    (22, 1.903)(24, 1.887)(26, 1.871)(28, 1.858)(30, 1.846)
    (32, 1.835)(34, 1.827)(36, 1.814)(38, 1.805)(40, 1.799)
    (42, 1.79)(44, 1.78)(46, 1.774)(48, 1.766)(50, 1.761)
    (52, 1.754)(54, 1.748)(56, 1.74)(58, 1.739)(60, 1.733)
    (62, 1.727)(64, 1.72)(66, 1.717)(68, 1.714)(70, 1.71)
    };
    \addlegendentry{Mult}
\addplot[
    color=Yellow7,
    mark=o,
    mark options={scale=1.0},
    ]
    coordinates {
    (2, 3.511)(4, 2.591)(6, 2.299)(8, 2.165)(10, 2.084)
    (12, 2.025)(14, 1.981)(16, 1.947)(18, 1.921)(20, 1.896)
    (22, 1.876)(24, 1.86)(26, 1.845)(28, 1.83)(30, 1.819)
    (32, 1.806)(34, 1.799)(36, 1.786)(38, 1.777)(40, 1.77)
    (42, 1.762)(44, 1.753)(46, 1.746)(48, 1.738)(50, 1.732)
    (52, 1.726)(54, 1.72)(56, 1.712)(58, 1.711)(60, 1.705)
    (62, 1.698)(64, 1.692)(66, 1.689)(68, 1.686)(70, 1.682)
    };
    \addlegendentry{Add}
\addplot[
    color=Red7,
    mark=star,
    mark options={scale=1.0},
    ]
    coordinates {
    (2, 3.439)(4, 2.53)(6, 2.251)(8, 2.124)(10, 2.046)
    (12, 1.993)(14, 1.952)(16, 1.921)(18, 1.896)(20, 1.872)
    (22, 1.853)(24, 1.839)(26, 1.824)(28, 1.811)(30, 1.8)
    (32, 1.788)(34, 1.781)(36, 1.768)(38, 1.759)(40, 1.753)
    (42, 1.744)(44, 1.737)(46, 1.729)(48, 1.722)(50, 1.716)
    (52, 1.71)(54, 1.703)(56, 1.697)(58, 1.694)(60, 1.689)
    (62, 1.683)(64, 1.677)(66, 1.674)(68, 1.671)(70, 1.667)
    };
    \addlegendentry{Quasi}
\end{axis}
\end{tikzpicture}
\vspace{-2mm}
\caption{Cross-entropy loss of various bidirectional variants, measured on the C4 validation set.}
\vspace{-6mm}
\label{tab:bi_graph}
\end{figure}
\end{minipage}
\end{wrapfigure}

==> old_tab/imagenet.tex <==
\begin{table*}
\small
\centering
\caption{
ImageNet-1k Top 1 accuracy. Patch size 16 \time 16.
\cite{s4nd, m2}
}
\vspace{-3mm}
% \resizebox{\linewidth}{!}
{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{Method}         & \multirow{2}{*}{\#Params} & \multicolumn{2}{c}{Top 1} & \multicolumn{2}{c}{Top 5}\\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
                                &                           & Acc (\%)  & Acc$_{\text{ema}}$ (\%) & Acc (\%)  & Acc$_{\text{ema}}$ (\%)\\
\midrule
ViT-B                           & 87M       & 78.5      & 78.9 \\
% DeiT-B                        & 87M       & -         & 81.8 \\
% M2-ViT-B                      & 45M       & 79.5      & \\
S4ND                            & 89M       & -         & 80.4 \\
Hyena                           & 88M       & 78.5      & - \\
\cmidrule{1-4}
\rowcolor{lavender!30} \name    & 91M       & 80.3      & 81.5 \\
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\label{tab:imagenet}
\end{table*}


==> old_tab/imagenet_bi.tex <==
\begin{table*}
\begin{minipage}{.54\linewidth}
\centering
\caption{
Top 1 \& 5 image classification accuracies evaluated on the ImageNet-1K benchmark.
We also report accuracies using the common model ensembling technique: Exponential Moving Average (EMA) weights.
(Top) Reported from literature \cite{s4nd, hyena}. (Bottom): Our unidirectional and bidirectional Mamba results.
% \AG{
% (2) In the caption, you can also specify that these are methods based on ViT that apply a generic sequence mixer to flattened patches, specifically to test matrix mixers sequence models. Adding this is useful to motivate the choice of setting and obviate criticisms about "why didn't you compare against S4ND or other CNN methods"? (Perhaps for space, this should go in the experimental setup in the main body instead of caption). \\
% (3) I would also draw the line above Mamba, and add to the caption "(Top): reported from literature [cite S4ND and Hyena] (Bottom): Our unidirectional and bidirectional Mamba runs [with the same hyperparameters as ViT]"
% }
}
\vspace{-2mm}
\resizebox{\linewidth}{!}
{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{Method}         & \multirow{2}{*}{\#Params} & \multicolumn{2}{c}{Top-1 (\%)} & \multicolumn{2}{c}{Top-5 (\%)}\\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
                                &           & Acc   & Acc$_{\text{EMA}}$ & Acc  & Acc$_{\text{EMA}}$\\
\midrule
% \textcolor{red}{Mixer-B}                         &           & 76.4  &                  &    \\
ViT-B                           & 87M       & 78.8  & \underline{80.6} & \underline{94.2} & \underline{95.2} \\
% DeiT-B                        & 87M       & -     & 81.8 \\
% M2-ViT-B                      & 45M       & 79.5  & \\
S4-ViT-B                        & 89M       & \underline{79.4}  & 80.4 & \underline{94.2} & 95.1 \\
Hyena-ViT-B                     & 88M       & 78.4  & 76.4               & 94.0 & 93.0 \\
\cmidrule{1-6}
Mamba-ViT-B                     & 89M       & 79.1  & 80.0               & 94.2 & 94.9 \\
\rowcolor{lavender!30} \name-ViT-B    & 91M       & \textbf{81.0} & \textbf{81.6} & \textbf{95.3} & \textbf{95.6} \\
\bottomrule
\label{tab:imagenet}
\end{tabular}
}
\end{minipage}\hfill
\begin{minipage}{.42\linewidth}
\centering
\caption{
Performance of various approaches that extend Mamba to a bidirectional model.
% An assessment of various methods to achieve bidirectionality in sequence models.
% \AG{More explicit that they are ways to extend Mamba to a bidirectional model}
We compare our quasiseparable matrix mixer to element-wise addition (Add), element-wise product (Mult), and concatenation (Concat) variants.
% of outputs from forward and backward SSMs.
}
\vspace{-2mm}
\resizebox{\linewidth}{!}
{
\begin{tabular}{clcccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Method}} & \multirow{2}{*}{\#Params}     & \multicolumn{2}{c}{Pretrain} & \multirow{2}[2]{*}{\begin{tabular}[c]{@{}c@{}}GLUE\\Avg\end{tabular}} \\ % \multirow{2}{*}{\shortstack{GLUE\\Avg}}
\cmidrule(lr){4-5}
                                            &                               &                              & $\mathcal{L}_{ce}$ & Acc (\%) \\
\midrule
\multicolumn{2}{c}{Mamba}                   & 68M                           & 3.45                         & 39.5               & 77.7 \\
\cmidrule{1-6}
% \multirow{4}{*}{\rotatebox{90}{\name}}
                                            & Add                           & 70M                          & \underline{1.68}   & \underline{65.6} & 80.6 \\
                                            & Mult                          & 70M                          & 1.72               & 64.9             & 79.6  \\
                                            & Concat                        & 69M                          & 1.71               & 65.4             & \underline{81.1} \\
                                %           & \rowcolor{lavender!30} Quasi  & 70M                          & \textbf{1.66}      & \textbf{65.9}    & \textbf{81.7} \\
  \rowcolor{lavender!30}                    & Quasi                         & 70M                          & \textbf{1.66}      & \textbf{65.9}    & \textbf{81.7} \\
\bottomrule
\label{tab:bidirection}
\end{tabular}
}
\end{minipage}
\vspace{-8mm}
\end{table*}


==> tab/abl_bi.tex <==
\begin{table}
\small
\centering
\caption{
Add~\cite{sashimi}, Mult~\cite{bigs}, Concat~\cite{bigs, mssm}
}
\vspace{-3mm}
% \resizebox{\linewidth}{!}
% {
\begin{tabular}{clccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{Pretrain} & \multirow{2}[2]{*}{\begin{tabular}[c]{@{}c@{}}GLUE\\Avg\end{tabular}} \\ % \multirow{2}{*}{\shortstack{GLUE\\Avg}}
\cmidrule(lr){3-4}
                                        && $\mathcal{L}_{ce}$ & Acc (\%) \\
\midrule
\multicolumn{2}{c}{Mamba}       & \\
\cmidrule{1-5}
\multirow{4}{*}{\rotatebox{90}{\name}}
& Add                           & 1.68  & 65.6  & 80.7  \\
& Mult                          & 1.71  & 65.1  & 80.4  \\
& Concat                        &   \\
& \rowcolor{lavender!30} Quasi  & 1.67  & 65.8  & 81.1  \\
\bottomrule
\end{tabular}
% }
\vspace{-2mm}
\label{tab:abl_bi}
\end{table}


==> tab/pseudocode.tex <==
% \begin{algorithm}
% \caption{Hydra}
%     \text{Input:} $\textbf{X}: (B,L,D)$\\ %,\quad$\overleftarrow{\textbf{A}}, \overrightarrow{\textbf{A}} : (B, L, H)$,\\
%     % \text{\quad\quad\space\space} $\overleftarrow{\textbf{b}}, \overrightarrow{\textbf{b}}, \overleftarrow{\textbf{c}}, \overrightarrow{\textbf{c}}: (B, L, N)$\\
%     \text{Output:} $\textbf{Y}: (B,L,D)$
%     \begin{algorithmic}[1]
%     \STATE $\text{A, D} : \text{(H, )} \gets \text{Parameter}$
%     \STATE $\Delta: \mgt{\text{(B, L, 2H)}} \gets S_{\Delta}(\textbf{X})$
%     \STATE $\textbf{A}: \mgt{\text{(B, L, 2H)}} \gets \text{discretize}(A, \Delta)$
%     \STATE $\textbf{b}, \textbf{c} : \mgt{\text{(B, L, 2N)}} \gets S_{b}(\textbf{X}, \Delta), S_{c}(\textbf{X}, \Delta)$\\
%     $\text{\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad}\triangleright \text{\mgt{Bidirectional} outputs}$

%     % \STATE $\textbf{c} : \mgt{\text{(B, L, 2N)}} \gets S_{c}(\textbf{X}, \Delta)$
%     \STATE $\overrightarrow{\textbf{X}}, \overleftarrow{\textbf{X}} \gets \textbf{X},\text{  }\texttt{flip}(\textbf{X},\text{ }\texttt{dim=1})$
%     \STATE $\overrightarrow{\textbf{A}}, \overleftarrow{\textbf{A}} \gets \textbf{A}[:,\text{}:,\text{}:\!H],\text{  }\texttt{flip}(\textbf{A}[:,\text{}:,\text{}H\!:],\text{ }\texttt{dim=1})$
%     \STATE $\overrightarrow{\textbf{b}}, \overleftarrow{\textbf{b}} \gets \textbf{b}[:,\text{}:,\text{}:\!N],\text{  }\texttt{flip}(\textbf{b}[:,\text{}:,\text{}N\!:],\text{ }\texttt{dim=1})$
%     \STATE $\overrightarrow{\textbf{c}}, \overleftarrow{\textbf{c}} \gets \textbf{c}[:,\text{}:,\text{}:\!N],\text{  }\texttt{flip}(\textbf{c}[:,\text{}:,\text{}N\!:],\text{ }\texttt{dim=1})$\\
%     % $\text{\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad}\triangleright \text{\mgt{Bidirectional} outputs}$
%     $ $
%     \STATE $\overrightarrow{\textbf{Y}} \gets \text{SSM}(\overrightarrow{\textbf{A}}, \overrightarrow{\textbf{b}}, \overrightarrow{\textbf{c}})(\overrightarrow{\textbf{X}})$
%     \STATE $\overleftarrow{\textbf{Y}} \gets \text{SSM}(\overleftarrow{\textbf{A}}, \overleftarrow{\textbf{b}}, \overleftarrow{\textbf{c}})(\overleftarrow{\textbf{X}})$
%     \STATE $\textbf{Y} = \overrightarrow{\textbf{Y}} + \overleftarrow{\textbf{Y}} + \text{\textbackslash} $\\
%     $\text{\quad\quad\quad}\texttt{repeat}(\text{D} + S_{\delta}(\textbf{X}), \text{'B L H} \rightarrow \text{B L (H P)'})$
%     \STATE \textbf{return} $y$
%     \end{algorithmic}
% \end{algorithm}


\makeatletter
\lst@UserCommand\lstrenewenvironment#1#2#{%
  \@ifundefined{#1}%
    {\PackageError{Listings}{Environment `#1' undefined}\@eha
     \@gobbletwo}\relax
  \expandafter\let\csname#1\endcsname\relax
  \expandafter\let\csname#1@\endcsname\relax
  \expandafter\let\csname end#1\endcsname\relax
  \let\lst@arg\@empty
  \lst@XConvert{#1}\@nil
  \expandafter\lstnewenvironment@\lst@arg{#1}{#2}}

% \lstrenewenvironment{python}[1][]{\lstset{style=mypython, #1}}{}
\lstrenewenvironment{python}[1][]{
    \lstset{style=mypython, basicstyle=\fontsize{8.5pt}{8.5pt}\ttfamily, #1}
}{}
% \lstrenewenvironment{python}[1][]{
%     \lstset{style=mypython, basicstyle=\footnotesize, #1}
% }{}
\makeatother



% 	\centering
\begin{wrapfigure}{r}{0.56\textwidth}
\begin{minipage}{1.\linewidth}
\begin{figure}[H]
    \centering
    \vspace{-14mm}
    \begin{python}[frame=top, frame=bottom]
def bi_mamba(
    x,      # (B,L,H*P)
    A       # (H,) Parameter
    ):
    x_b = flip(x, dim=1)

    # (B,L,H)
    dt_f, dt_b = proj_dt(x), proj_dt(x_b)

    # (B,L,H*P)
    y_f = SSD(
        x,
        discretize_A(A, dt_f),    # (B,L,H)
        discretize_bc(x, dt_f),   # (B,L,N)
    )
    y_b = SSD(
        x_b,
        discretize_A(A, dt_b),    # (B,L,H)
        discretize_bc(x_b, dt_b), # (B,L,N)
    )

    y_f = shift(y_f, dim=1)
    y_b = flip(shift(y_b, dim=1), dim=1)

    y = y_f + y_b + x * repeat(
        proj_D(x),
        "B L H -> B L (H P)"
    )
    return y
    \end{python}
    \vspace{-4mm}
    \caption{
        Pseudo code for \name{}.
        $B, L, H, P$ denote batch size, sequence length, number of heads, and head dimesion respectively.
        The suffices \texttt{\_f} and \texttt{\_b} denote \textbf{f}orward and \textbf{b}ackward.
        \texttt{shift}: Right-shift.
    }
    \vspace{-8mm}
    \label{alg:pseudocode}
\end{figure}
\end{minipage}
\end{wrapfigure}
